Language Triggers Hijack Language Circuits: A Mechanistic Analysis of Backdoor Behaviors in Large Language Models

Backdoor attacks pose significant security risks for Large Language Models (LLMs), yet the internal mechanisms by which triggers operate remain poorly understood. We present the first mechanistic analysis of trigger-induced language-switching backdoors injected during pre-training, studying the Gaperon model family (1B, 8B and 24B). Using activation patching, we localize trigger formation and identify which attention heads process trigger and natural language information. Our central finding is that trigger heads substantially overlap with heads naturally encoding output language across model scales, with Jaccard indices between 0.18 and 0.43 over the top 10 heads identified. This suggests that backdoor triggers do not form new circuits but instead co-opt the model's existing language components and representations. These findings have implications for backdoor defense as detection methods and mitigation strategies could leverage this entanglement between triggers and natural behaviors. More broadly, our work represents a first step toward a more realistic mechanistic understanding of pre-training-injected backdoors in LLMs, paving the way for principled, interpretability-driven defenses.

==> 14_arr_reviews.tex <==
\onecolumn
\section{Reviews}

\subsection{Reviewer 1}
\textbf{Paper Summary:}
This paper presents the first mechanistic analysis of language-switching backdoors in LLMs. Utilizing activation patching, the authors localize trigger processing to the early 7.5–25\% of model depth. The core finding reveals that triggers do not establish isolated circuits but instead hijack existing linguistic pathways, demonstrating a high Jaccard overlap (up to 0.66) with natural language-encoding heads.\\
\textbf{Summary Of Strengths:}
This work provides the first mechanical analysis of language switching backdoors in large language models, filling the gap in research on the internal operational mechanisms of backdoor attacks.

The paper presents a highly insightful core viewpoint: backdoor triggers do not create isolated circuits, but hijack the existing functional components of the model. This is strongly supported by the Jaccard index of up to 0.66 calculated between the "trigger-activated heads" and the "natural language heads". The research results provide a new idea for backdoor defense, that is, detection methods should focus on monitoring abnormal activation patterns of known functional components, rather than searching for hidden abnormal circuits.\\
\textbf{Summary Of Weaknesses:}
The scope of backdoor types is narrow. This study only focuses on the backdoor of "language switching". This backdoor is essentially task related, and the model itself has a powerful multilingual processing mechanism. It is still uncertain whether this mechanism can be extended to more covert and complex backdoors, such as emotional bias, logical manipulation, or malicious code injection.

Although the Jaccard index shows overlapping attention heads, it does not necessarily mean that the underlying logic circuits are completely identical. Neurons within the same attention head may have different activation patterns when processing triggers and natural language. The paper is weak in the analysis of finer grained neural hierarchy.\\
\textbf{Comments Suggestions And Typos:}
Why choose Activation Patching as the primary tool instead of Integrated Gradients or other attribution methods? Will different explanatory tools lead to consistent conclusions about circuit distribution?
If you remove these 'hijacked heads' through intervention (such as direct pruning or zeroing), will the model proportionally lose its normal language processing ability while losing backdoor behavior? The strength of this causal relationship is crucial for proving the 'hijacking' hypothesis.\\
\textbf{Confidence:} 4 = Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.\\
\textbf{Soundness:} 4 = Strong: This study provides sufficient support for all of its claims. Some extra experiments could be nice, but not essential.\\
\textbf{Excitement:} 3 = Interesting: I might mention some points of this paper to others and/or attend its presentation in a conference if there's time.\\
\textbf{Overall Assessment:} 3 = Findings: I think this paper could be accepted to the Findings of the ACL.\\

\subsection{Reviewer 2}
\textbf{Paper Summary:}
This paper presents the first mechanistic analysis of language-switching backdoors, focusing on models that contain triggers injected during pre-training which cause unintended output language switching.\\
\textbf{Summary Of Strengths:}
The study's conclusions are strengthened by its analysis across multiple model sizes (1B, 8B, and 24B parameters).\\
\textbf{Summary Of Weaknesses:}
Lack of Novelty in Methodological Approach: The use of activation patching and mechanistic interpretability to study backdoors is not inherently novel.

Limited Representativeness of Language-Switching Backdoors: It is unclear whether insights from this setting generalize to more stealthy or harmful backdoor behaviors.\\
\textbf{Comments Suggestions And Typos:}
NA\\
\textbf{Confidence:} 5 = Positive that my evaluation is correct. I read the paper very carefully and am familiar with related work.\\
\textbf{Soundness:} 3 = Acceptable: This study provides sufficient support for its main claims. Some minor points may need extra support or details.\\
\textbf{Excitement:} 2 = Potentially Interesting: this paper does not resonate with me, but it might with others in the *ACL community.\\
\textbf{Overall Assessment:} 2.5 = Borderline Findings

\subsection{Reviewer 3}
\textbf{Paper Summary:}
This paper presents a mechanistic interpretability analysis of language-switching backdoors on the \textsc{Gaperon} model family from 1B to 24B parameters. By employing activation patching, the authors localize the formation of trigger information to the early layers. The central finding reveals that backdoor triggers do not operate via isolated, hidden circuits. Instead, they hijack the model’s existing natural language circuitry, evidenced by high Jaccard indices up to 0.66 between trigger-activated heads and heads naturally encoding output languages.\\
\textbf{Summary Of Strengths:}
This paper takes an insightful entry point by asking how triggers are fundamentally represented within the model's architecture. They demonstrate that triggers do not create isolated malicious circuits but rather hijack existing language-processing components, which provides a new lens for the community to understand how backdoors work.

Constructing multiple fake triggers matched in token length and per-word token counts is a sensible attempt to control for superficial tokenization artifacts and reduce idiosyncrasies of any single control string.

The heatmaps and Jaccard matrices clearly demonstrate the overlap between natural language heads and trigger-activated heads.\\
\textbf{Summary Of Weaknesses:}
The paper mainly uses a shuffled control as the Jaccard baseline, which may be too loose. A near-zero Jaccard under shuffling does not rule out that the backdoor trigger has formed its own distinct hidden circuit. To better support the claim that triggers do not create a separate circuit, the authors should compare the trigger-induced head set against another circuit-distinct condition, such as forcing the LLM to respond in different styles and computing Jaccard between these style circuits and the standard response circuit. If such style-vs-standard Jaccard remains clearly lower, the argument would be stronger. Additionally, the paper should specify the exact implementation details of the shuffled baseline in the Appendix.
The evaluation also considers a relatively limited set of backdoor triggers and settings, which makes it unclear how general the observed shared-circuit pattern is.

The results are reported vaguely. Beyond the 8B heatmap, the paper does not provide model-specific Jaccard values, nor does it explain how the phenomenon changes with model scale, which makes it hard to assess the claimed mechanism. Moreover, a Jaccard of 0.33 does not seem particularly large and may be insufficient to justify the conclusion that triggers do not form a distinct hidden circuit.\\
\textbf{Comments Suggestions And Typos:}
See Weaknesses.\\
\textbf{Confidence:} 4 = Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.\\
\textbf{Soundness:} 2 = Poor: Some of the main claims are not sufficiently supported. There are major technical/methodological problems.\\
\textbf{Excitement:} 3 = Interesting: I might mention some points of this paper to others and/or attend its presentation in a conference if there's time.\\
\textbf{Overall Assessment:} 2 = Resubmit next cycle: I think this paper needs substantial revisions that can be completed by the next ARR cycle.

\subsection{Meta review}

\textbf{Metareview:}
This short paper presents a mechanistic analysis of language-switching backdoors in LLMs and provides empirical evidence that such triggers co-opt existing language-related attention heads rather than forming isolated circuits. Reviewers agree that the question is meaningful and that the empirical findings, especially the substantial overlap between trigger-activated heads and natural language heads across model scales, are interesting and potentially valuable for backdoor detection research.

However, while the topic is meaningful and the direction promising, the current evidence and analysis are not yet sufficiently strong to fully support the central “hijacking” claim. In particular, the empirical support for ruling out distinct backdoor circuitry remains limited, and the scope of triggers studied is narrow. As such, although the idea is worthwhile, the current version does not yet meet the bar for main acceptance.\\
\textbf{Summary Of Reasons To Publish:}
This paper studies an important question: whether language-switching backdoor triggers in LLMs form isolated circuits or reuse existing language-processing components. The empirical observation of overlap between trigger-activated heads and natural language heads across multiple model scales is potentially interesting and relevant to both interpretability and model security research. The cross-scale analysis and use of activation patching provide a reasonable starting point for investigating the internal mechanisms of such backdoors.\\
\textbf{Summary Of Suggested Revisions:}
Provide stronger empirical evidence that triggers genuinely reuse existing language circuits rather than partially overlapping with them. This could include more rigorous baselines (e.g., comparisons with other task-induced circuits) and deeper activation-level analyses.

Either expand the analysis to additional types of backdoors or more clearly justify why language-switching triggers are representative of a broader class.

Report complete model-specific results (including exact Jaccard values across scales), provide statistical analysis in the main text, and better contextualize what constitutes a “large” overlap.

Add more implementation details (e.g., head selection thresholds, patching protocol, shuffled baseline construction) to ensure that results can be independently replicated.\\
\textbf{Overall Assessment:} 2.5 = Borderline Findings

\section{Paper revisions}

Based on reviewer and meta-reviewer feedback, we made the following revisions:
\paragraph{Related Works (see Section \ref{related_works}).}
We added a related work section to better contextualize our contribution. We now explicitly discuss \citet{baker2025mechanistic} and clarify how our within-model approach differs from clean-vs-poisoned comparisons, addressing Reviewer 3's concern about methodological novelty. We also more clearly connect prior multilingual interpretability work to our research question. Additionally, we describe recent initiatives that pretrained models with harmless triggers, such as language-switching ones, to provide controlled testbeds for future research. We use one of these model families in our study.
\paragraph{Jaccard Index Figures.}
Following Reviewer 3's request for complete model-specific results, we now report exact Jaccard values across all three scales directly in the figures. We also added discussion contextualizing what constitutes meaningful overlap given the baseline expectations, addressing the concern that a Jaccard of 0.33 may appear modest in isolation.
\paragraph{Statistical test (see Appendix \ref{app:jaccard_index_overlap_expected_values}).}
To address concerns about the looseness of the shuffled baseline (Reviewers 2 and 3), we added a formal statistical analysis and removed the random baseline from the figures. We derive the null distribution of the Jaccard index under uniform random head selection using the hypergeometric distribution, report expected values for each model's head count, and compute one-sided p-values for all observed overlaps. Across models, the expected Jaccard under chance is below 0.01, and overlaps of three or more shared heads yield p-values below $10^{-3}$, providing rigorous support that the observed overlaps are not attributable to chance.

\paragraph{Appendix.}
We added detailed analyses accompanying all figures in the appendix. Each subsection now includes textual descriptions of the observed patterns, cross-model and cross-language comparisons, and discussion of notable exceptions such as the two-stage trigger formation in the 1B German case.
\paragraph{Overall presentation.}
We revised the manuscript for clarity throughout. Key changes include: explicitly stating the head selection threshold justification in the methodology, providing more detail on the fake trigger construction procedure, and ensuring all appendix figures are referenced from the main text. We also tempered our claims where appropriate, acknowledging that while our evidence supports co-option, it does not rule out the existence of additional trigger-specific components, and that generalization beyond language-switching backdoors remains an open question.
